Predictable Verification using Intrinsic Definitions

We propose a novel mechanism of defining data structures using intrinsic definitions that avoids recursion and instead utilizes monadic maps satisfying local conditions. We show that intrinsic definitions are a powerful mechanism that can capture a variety of data structures naturally. We show that they also enable a predictable verification methodology that allows engineers to write ghost code to update monadic maps and perform verification using reduction to decidable logics. We evaluate our methodology using Boogie and prove a suite of data structure manipulating programs correct.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}




==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}

Hoare triples of the form $t=\{\alpha\} s \{\beta\}$ are often compiled to pure logical formulas called verification conditions $VC_t$ such that the Hoare triple $t$
is valid iff $VC_t$ is valid. When verifying programs manipulating data structures, these 
Hoare triples typically have preconditions $\alpha$ that assume that certain pointers point to certain data structures (like say binary search trees or linked lists with certain properties like being sorted), and the postcondition asks whether such data structure properties are \emph{maintained} after the destructive updates the program $s$ performs on the heap. The verification condition $VC_t$ hence has a special form--- rather than asking whether complex properties of data structures emerge with the program's execution, the condition asks whether properties of structures are \emph{maintained} by the program.


This work is founded on the intuition that establishing \emph{maintenance} of properties of structures can be much easier than reasoning with general properties of structures. In particular, as we will show in this work, we can verify the maintenance of properties using \emph{decidable logics} based on quantifier-free reasoning while their counterparts for general logic reasoning is typically undecidable as it requires reasoning with quantifiers and reasoning with recursive definitions using induction. 

Data structures embedded in the heap are typically represented using their properties, which are in turn described using recursion and quantification. 
When even a small part of the data structure changes due to mutation, we need to reestablish the properties of the data structure, which typically requires induction. The goal of this work is to reestablish properties of data structures using a much simpler style of reasoning, which in particular is decidable reasoning.

Our key idea is to use a class of \emph{monadic functions} with \emph{local constraints} to establish properties of data structures. Give a heap with a set of locations $L$, monadic functions are maps $f: L \rightarrow D$, where $D$ is some domain. Typical domains include the set of locations $L$ itself, the set of natural numbers, the set of integers, the set of real numbers, the set of subsets of integers, etc. Furthermore, a constraint on a set of monadic functions $\{f_1, \ldots, f_n\}$ is of the form 
$\forall x \in L: \varphi(x, f_1, \ldots, f_n)$, where $\varphi$ is quantifier-free. The formula $\varphi$ can mention any term constructed from $x$, followed by poi

